Learning 3D-3D Correspondences for One-shot Partial-to-partial Registration

While 3D-3D registration is traditionally tacked by optimization-based methods, recent work has shown that learning-based techniques could achieve faster and more robust results. In this context, however, only PRNet can handle the partial-to-partial registration scenario. Unfortunately, this is achieved at the cost of relying on an iterative procedure, with a complex network architecture. Here, we show that learning-based partial-to-partial registration can be achieved in a one-shot manner, jointly reducing network complexity and increasing registration accuracy. To this end, we propose an Optimal Transport layer able to account for occluded points thanks to the use of outlier bins. The resulting OPRNet framework outperforms the state of the art on standard benchmarks, demonstrating better robustness and generalization ability than existing techniques.

==> figure/partial_visible.tex <==
\begin{figure}[t]
    \includegraphics[width=2.65cm]{image/piano.png}
    \includegraphics[width=2.65cm]{image/person.png}
    \includegraphics[width=2.65cm]{image/airplane.png}
    \includegraphics[width=2.65cm]{image/stool.png}
    \includegraphics[width=2.65cm]{image/cup.png}
    \caption{\label{5_obj} Visualization of the alignments and correspondences obtained with our approach in the self-occlusion scenario. We plot the point sets (source in blue, target in orange) after alignment, but shifted horizontally for clarity. The green lines in the bottom row depict the correspondences found with our approach.
    %From left to right, piano, person, airplane, stool and cup. The source point cloud is represented in the orange color. The target point cloud is represented in the blue color. We transform the target point cloud to the source point cloud position using our network estimated pose. As you can see, the target point cloud perfectly match the source point cloud.
    }
\end{figure}
